Finsler Geometry, Spacetime & Gravity -- From Metrizability of Berwald Spaces to Exact Vacuum Solutions in Finsler Gravity

This PhD dissertation covers a range of topics in Finsler geometry and Finsler gravity, most notably: (i) the characterization of Berwald spaces, (ii) pseudo-Riemann (non-)metrizability of Berwald spaces, (iii) $(\alpha,\beta)$-metrics, (iv) exact solutions to Pfeifer and Wohlfarth's vacuum field equation in Finsler gravity, and (v) Finsler gravitational waves and their observational signature. An extended abstract can be found in the dissertation itself.

==> Preface.tex <==
% \section{Preface}

% We investigate exact vacuum solutions to the field equation in Finsler gravity. We focus largely on geometries of $(\alpha,\beta)$-metric type, and in particular Randers and $m$-Kropina metrics.

==> curriculumVitae.tex <==
% Version 1.0 by Joos Buijs, Eindhoven, August 2014
% Use at your own risk.
% Attribution is appreciated 
\cleardoublepage
\phantomsection
\addcontentsline{toc}{chapter}{About the Author}
\chapter*{About the Author}
\fancyhead{}
\fancyhead[RE]{\textit{About the Author}}
\fancyhead[LO]{\textit{About the Author}}
%\pagestyle{empty}

%\color{red}
Sjors Heefer was born on February 24, 1994 in 's-Hertogenbosch, the Netherlands.
After finishing his Dutch VWO high school degree in 2012 at the ds.~Pierson College in 's-Hertogenbosch% (VWO is the Dutch abbreviation for `preparatory scientific education')
, he went on to study Physics and Astronomy at Radboud University, Nijmegen, the Netherlands. Here he obtained his BSc degree in 2016 and his MSc degree in 2019, specializing in mathematical physics and graduating within the quantum gravity group with a master's thesis titled:  \textit{Advancements on the Covariance of the $\kappa$-Poincar\'e Model and Relative Locality}. In 2018 he started his PhD-TA at Eindhoven University of Technology, Department of Mathematics and Computer Science; a special five-year position combining PhD research with a considerable amount of teaching responsibility. His research has mainly focused on Finsler geometry and its application to gravity and spacetime. The results are presented in this dissertation. During his time as a PhD student, Sjors also obtained his university teaching qualification (UTQ). Moreover, after having been nominated twice, he won the award \textit{Best teacher Applied Physics year 2} for his lectures given for the course \textit{General Relavitity}. As of November 2023, he has been employed as a lecturer at the Department of Mathematics and Computer Science, Eindhoven University of Technology.

\newpage
